Throughput and range characterization of IEEE 802.11ah

The most essential part of Internet of Things (IoT) infrastructure is the wireless communication system that acts as a bridge for the delivery of data and control messages. However, the existing wireless technologies lack the ability to support a huge amount of data exchange from many battery driven devices spread over a wide area. In order to support the IoT paradigm, the IEEE 802.11 standard committee is in process of introducing a new standard, called IEEE 802.11ah. This is one of the most promising and appealing standards, which aims to bridge the gap between traditional mobile networks and the demands of the IoT. In this paper, we first discuss the main PHY and MAC layer amendments proposed for IEEE 802.11ah. Furthermore, we investigate the operability of IEEE 802.11ah as a backhaul link to connect devices over a long range. Additionally, we compare the aforementioned standard with previous notable IEEE 802.11 amendments (i.e. IEEE 802.11n and IEEE 802.11ac) in terms of throughput (with and without frame aggregation) by utilizing the most robust modulation schemes. The results show an improved performance of IEEE 802.11ah (in terms of power received at long range while experiencing different packet error rates) as compared to previous IEEE 802.11 standards.

==> Section4.tex <==
\section{Conclusions}
\label{Conclusions}
In this paper, we provide a comparison between IEEE 802.11ah and current IEEE 802.11a/n/ac in terms of range and throughput. Detailed results indicate that IEEE 802.11ah benefits from the widest coverage, due to the lower frequency band, a narrower bandwidth and a more robust coding scheme. It shows, at least, a fivefold increase with respect to the second best range (IEEE 802.11a), and more than ten times improvement with regard to the worst case (IEEE 802.11n in the 2.4GHz band). On the other hand, IEEE 802.11ah presents the lowest throughput, in comparison with other amendments; a maximum throughput of 144kbps (reduced to 71kbps when \textit{PER} = 50\%) can be achieved at the limits of its estimated coverage, which is enough for the use cases this technology is targeting. Given the use case scenarios where the size of data frames is inherently small, the use of aggregation slightly mitigates the excess of overhead but its impact is limited by the low data rates that 802.11ah devices will support. In our future work, we plan to extend our comparison by means of simulations of more complex scenarios.
